Fitting Square Pegs Through Round Pipes: Unordered Delivery Wire-Compatible with TCP and TLS

Internet applications increasingly employ TCP not as a stream abstraction, but as a substrate for application-level transports, a use that converts TCP's in-order semantics from a convenience blessing to a performance curse. As Internet evolution makes TCP's use as a substrate likely to grow, we offer Minion, an architecture for backward-compatible out-of-order delivery atop TCP and TLS. Small OS API extensions allow applications to manage TCP's send buffer and to receive TCP segments out-of-order. Atop these extensions, Minion builds application-level protocols offering true unordered datagram delivery, within streams preserving strict wire-compatibility with unsecured or TLS-secured TCP connections. Minion's protocols can run on unmodified TCP stacks, but benefit incrementally when either endpoint is upgraded, for a backward-compatible deployment path. Experiments suggest that Minion can noticeably improve performance of applications such as conferencing, virtual private networking, and web browsing, while incurring minimal CPU or bandwidth costs.

==> 6minion.tex <==
\section{An IPv6 Minion}
\label{sec:6minion}

Why v6 minion: when negotiating, provides a deployment path to IPv6,
since new transports would much rather be running directly on top of IPv6.

(short section)

==> arguments.tex <==
\section{Why Not UDP Encapsulation?}
\label{sec:arguments}

Given that the demand for new transport services exists,
new transport services are being built and deployed on top of UDP.
Applications such as
Internet telephony (Skype),
video streaming (Adobe's RTMFP for Flash), and
bulk background transport (Bittorrent's uTP),
continue to build their own 
narrowly-focused
transport services over UDP,
and deploy them as part of the application.
To encourage deployment,
transports designed at the IETF
are also employing UDP encapsulation to navigate NATs in the network%
~\cite{tuexen10udp, phelan10dccp}.
While the idea of UDP encapsulation seems seductively simple,
this section discusses
why {\em simple} UDP encapsulation of a new transport
is an inadequate and fragile solution that may
lead to more network encumbrances in the long term.

\subsection{A Taxonomy of Transport Functions}
To understand
how UDP encapsulation fits in the larger picture of
middlebox traversal,
we examine the
interactions between middleboxes
and the traditionally-end-to-end transport layer.
We first factor out functional components 
within the traditional transport layer into four sub-layers,
as previously proposed in \Tng~\cite{ford08breaking}.
Starting from the sub-layer immediately above the network layer, 
these are:
\begin{description}
\item [The Endpoint Layer] factors out communication endpoint information---%
  port numbers in the current Internet architecture---%
  that policy-enforcing middleboxes such as firewalls, NATs,
  and traffic shapers require for operation;
\item [The Flow Regulation Layer]  
  factors out congestion control and other functions
  that may require network interaction
  for purposes of adapting to network heterogeneity;
\item [The Semantic Layer] 
  factors out application-oriented services
  such as end-to-end reliability and ordering; and
\item [The Isolation Layer]
  is an optional layer,
  traditionally above the Semantic Layer,
  which provides end-to-end cryptographic security
  via protocols such as TLS~\cite{rfc5246} and DTLS~\cite{rfc4347}.
\end{description}

Figure~\ref{f:layers-middleboxes} shows how middleboxes interact
with and interpose on different transport layer components.
NATs and Firewalls 
care about port numbers and application endpoint information,
Performance Enhancing Proxies (PEPs)~\cite{rfc3234} 
care about congestion control,
Traffic Normalizers~\cite{handley01network}
use detailed information about the TCP state machine to 
thwart network attacks,
and Corporate Firewalls are increasingly starting to employ
SSL proxies as trusted intermediaries to
prevent attacks through encrypted channels~\cite{marko10using}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-middleboxes.eps}
\caption{A taxonomy of Transport functions showing how middleboxes interact with the Transport}
\label{f:layers-middleboxes}
\end{figure}


\subsection{Network Considerations}

Figure~\ref{f:layers-current-transports} 
shows how transports are designed and deployed on the Internet,
and a comparison with Figure~\ref{f:layers-middleboxes}
shows how new transports conflict with legacy middleboxes.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-current-transports.eps}
\caption{Transport protocols in the Tng taxonomy}
\label{f:layers-current-transports}
\end{figure}

While NATs and firewalls often support both TCP and UDP,
they support TCP flows more efficiently
due to the connection state information it provides.
Since NATs cannot precisely determine a UDP session's lifetime,
an application wishing to keep a UDP connection alive
across a NAT or firewall must send keepalive packets
at least every two minutes~\cite{rfc4787},
whereas idle TCP connections require keepalives 
only once every two hours~\cite{rfc5382}.
TCP thus has practical advantages in both bandwidth and power consumption,
especially important for mobile devices,
which are frequently located behind NATs and firewalls
and must keep connections open to listen for incoming notifications.

While simple home NATs and Firewalls
care mainly about port numbers (application endpoint information),
significant parts of the Internet
are behind more sophisticated middleboxes~\cite{rfc3234}
which use TCP connection state information
and assume TCP mechanisms,
such as ack clocking and flow control to achieve their ends.

Stateful Firewalls
maintain and use connection state for filtering traffic and to avoid attacks.
TCP's connection-oriented state machine
makes this information easily available.
Since UDP is connectionless,
Stateful Firewalls
use non-trivial methods
such as 
Deep Packet Inspection (DPI)
and rely on arbitrary timeouts 
and ICMP messages
to determine the state of a session that uses UDP~\cite{northcutt05inside},
thus creating disincentives for operators to allow UDP traffic
into their networks.

Traffic Normalizers~\cite{handley01network}
use detailed information about the TCP state machine to 
thwart network attacks,
and Corporate Firewalls increasingly employ
SSL proxies as trusted intermediaries to
prevent attacks through encrypted channels~\cite{marko10using}.
Using UDP leads to heavy use of DPI,
since both Firewalls and Traffic Normalizers
have less information to work with than they would have with TCP,
and they are thus heavily incentivized against allowing UDP traffic.

A new transport that runs on UDP
appears as one among the plethora of extant applications 
that use UDP,
and thus will not be able to navigate broad sledgehammer-like firewall rules 
often found in corporate (and often hotel) firewalls 
that disallow any incoming UDP traffic.

PEPs~\cite{rfc3234}
improve TCP flow performance over 
unconventional network paths,
such as lossy wireless or satellite links,
often by intervening in
TCP mechanisms such as
flow control and ack clocking.
PEPs ignore UDP traffic,
and consequently transports
such as SCTP, SST, and DCCP,
that use TCP-like congestion control mechanisms,
appear to perform poorly on these paths
when run atop UDP.

All these middleboxes 
need to be made aware of a new transport
for the transport to be deployable and performant in the network
on top of UDP.

\subsection{Yet Another Layer of Multiplexing}
%A more subtle point is worth making
%about stacking transport protocols
%atop UDP.
Current proposals~\cite{tuexen10udp, phelan10dccp}
use UDP port numbers merely to demultiplex 
the new transport protocol on top;
the identity of 
the communicating endpoints is hidden away 
in a {\em new} set of port number fields (separate from the UDP port numbers)
embedded in the new transport's protocol headers.
There are thus two sets of port numbers
at the ends:
the UDP port numbers are used to identify
the transport protocol---%
e.g., UDP port 9899 indicates SCTP atop UDP---%
plus the inner transport's SCTP port numbers,
used to identify the application process.
The UDP port numbers are thus 
not usable as a basis for identifying end-applications,
as is commonly done at firewalls.
As a result,
while this solution works for NATs,
Firewalls will need to understand the new protocol's interior headers
to enforce network policy based on port numbers,
and until they are able to, 
administrators will be tempted simply to block the new transport's UDP port.
Thus, where an HTTP session over TCP works,
an HTTP session over SCTP/UDP will not,
even if the firewall's policy is intended to allow web traffic in general.

Future generations of firewalls may eventually understand the 
inner transport and enforce policy 
based on the inner transport's port numbers,
but this simply brings us  back to where we started,
with devices in the network ``understanding''
and allowing traffic from a relatively static
and difficult-to-evolve set of transports atop IP.

Proposals for UDP encapsulation of new transports%
~\cite{tuexen10udp, phelan10dccp}
miss the point that middleboxes need endpoint information,
and encapsulating that information does more harm by 
triggering an arms race with firewall providers.

\subsection{End Host Considerations}

%User-space transports are much easier to deploy
%than kernel-space transports.
Getting user-space transport implementations to perform competitively
with kernel-space implementations
is a non-trivial issue,
and requires much more low-level access than 
is available to most applications 
for close to kernel-level performance~\cite{edwards95experiences}.
Ack-clocked transports,
such as SCTP and SST,
rely on tight timing in transmission and delivery of acks.
Coalescence of ack- and data-delivery,
which results from poor interaction between the ack-clocking of data
and process scheduling on the endhosts,
leads to increased burstiness in the transport~\cite{prasad04effects},
breaking TCP's self-clocking mechanism~\cite{jacobson88congestion},
and resulting in poor performance of TCP-like congestion control%
~\cite{zec02estimating}.
Deploying highly performant transports 
on top of UDP is difficult,
and bandwidth intensive applications
will tend to opt for TCP, 
despite its strait-jacketed service options,
for performance reasons.

Further, new transports that use delay-based congestion control mechanisms
will simply not work in user-space
due to the increased noise in delay signals that comes with
data copying across
the kernel-user boundary 
and with context-switching latency.

\com{
\subsection{Deployment Timescales}
Application requirements and code can and do change more often 
than endhost kernels and code,
which are orders of magnitude faster than changes in the network.
(XXX Quantify through examples. 
changes in killer apps in the last ten years---
web to chat to p2p to games to Internet telephony to Internet video and TV---
changes to network stacks,
changes in the network in the last ten years---ECN deployment?.)
An attempt to deploy a new general-purpose transport protocol,
such as SCTP or SST,
must generally span these three timescales,
which is a very difficult proposition.
}

\subsection{Legacy Comes With Benefits Too}

TCP implementations have 
been maturing and optimized over the past 2-3 decades,
and detailed instrumentation is available for 
learning from and tweaking TCP stacks~\cite{web100, gunawi04deploying}
Offloading parts of the TCP engine
is becoming increasingly important and relevant
~\cite{mogul03tcp},
improving TCP performance and efficiency in high-speed networks.

While other parts have been difficult to get deployed,
variants to the original TCP congestion control~\cite{jacobson88congestion}
are commonplace in general-purpose OS kernels---%
likely in large part due to the fact that congestion control modifications
can usually be deployed without wire-format modifications to TCP.
The major general-purpose Operating Systems---%
MacOSX, Windows7, and Linux---%
all use 
very different congestion control algorithms:
TCP NewReno, Compound TCP, and CUBIC TCP, respectively.
As of kernel v2.6.13, Linux has made it easy for a user 
to choose from a number of congestion control alternatives in the kernel
at run-time%
\footnote{{\em ls /lib/modules/`uname -r`/kernel/net/ipv4/} on a
  Linux-2.6.34 system shows
  an impressive 11 distinct TCP congestion control mechanisms available
  as kernel modules.},
and Mac OSX allows enabling and disabling TCP variants 
such as NewReno and SACK through {\em sysctl}s.
Kernel mechanisms for plugging different
congestion control variants for TCP
already exist in popular Operating Systems,
and where they do not exist yet,
they represent a worthy goal
for kernels that are already dealing with 
diverse network conditions 
ranging from 
low-bandwidth and lossy cellular connectivity on mobile and handheld devices 
to
high-bandwidth connectivity on desktops within enterprise networks.

Legacy TCP thus comes with
a performant and functionality-rich body of software artifacts and tools,
as well as widespread human experience in the industry,
which generally outweighs the costs
of deploying and performance-tuning a new transport atop UDP.

%  SCTP ships with FreeBSD,
%  DCCP is a compile-able option in FreeBSD,
%  and both SCTP and DCCP are compile-able options in Linux.

%In summarizing the previous section
%\begin{enumerate}
%\item Demand exists for new transport services.
%\item Performance issues with deploying new transport in userspace on UDP
%\item Accurate timing and heavy perf optimization with network hardware 
%and middleboxes heavily incentivizes using TCP over any other transport 
%for data- and throughput-intensive applications.
%\item CC changes are easy to deploy in-kernel, where timing is also better
%for RTT- and delay-based CC, such as in CompoundTCP and TFRC.
%\end{enumerate}

\com{
\subsection{Moving Forward:  }
To break out of this transport logjam, 
our goals are to build new transport services,

we therefore argue that the following goals are necessary.
\begin{enumerate}
\item Provide new general-purpose services,
such as 
multi-streaming,
and message-oriented delivery.
\item Require minimal changes to the kernel, to reduce deployment hurdles,
and no changes to middleboxes.
\end{enumerate}

The following supplementary goals are corollaries:
\begin{enumerate}
\item Utilize TCP congestion control for compatibility with PEPs.
\item Provide incremental deployment paths for 
endhost-only kernel modifications.
\item Expose different levels of abstraction within 
the traditional transport layer,
so that special-purpose transports 
can employ existing code for the parts that they want to reuse.
(do we need this goal?  overlaps with much previous work, see icTCP.)
\end{enumerate}
}

\com{
Our proposal is to
treat TCP in kernel as 
a protocol that can be used for getting
through the network, 
for ack clocking the,
and for congestion control,
and to let applications deploy services 
in userspace
on top of these functions.
}


==> cm.tex <==
\subsection{A Poor Man's Congestion Manager}
\label{sec:cm}

The Congestion Manager~\cite{balakrishnan99integrated}
provides a framework by which all application flows 
between two endhosts 
share congestion state,
irrespective of the transport protocol they use.
The Congestion Manager sits as a shim between IP and the transport layers,
and implements congestion control for all the transport protocols.

Since \ucobs and \utls offer
a congestion-controlled and reliable datagram interface,
we can also use them as the basis for 
a Poor Man's Congestion Manager (PM-CM)
that provides aggregate congestion control to
\utcp-based transports above.
Between two endhosts using PM-CM,
applications that use a \utcp-based transport
can automatically share a single \utcp flow underneath,
thereby sharing congestion state.
A PM-CM shim atop \ucobs or \utls
introduces a thin header, 
similar to the CM,
to multiplex and demultiplex
different application flows.


==> dccp.tex <==
\subsection{A Poor Man's DCCP}
\label{sec:dccp}

The Datagram Congestion Control Protocol (DCCP)~\cite{rfc4340, kohler06dccp}
was designed for streaming and voice/video-conferencing applications,
and it provides a congestion-controlled unreliable datagram service
with the ability to negotiate congestion control mechanisms at 
flow setup time.

By definition,
\ucobs and \utls
provide the semantic equivalent of
DCCP with TCP-like congestion control~\cite{rfc4341},
with the difference that DCCP does not provide reliability.

Providing negotiable congestion control atop \utcp, 
while not readily available, can be designed.
As a first step, more congestion control variants
need to be made available for TCP within popular OSes, 
and need to be made pluggable---%
Linux-2.6.34 provides an impressive $11$ congestion control
modules for TCP,
but the choice of a module currently applies system-wide,
and not flow-specific,
as would be required for PM-DCCP.

With congestion control options available in the TCP-stack,
PM-DCCP can negotiate,
above \utcp,
congestion control methods to be used
in the flow,
and use flow-level controls (such as a socket option)
to use the appropriate congestion control method for the flow.
The underlying \utcp flow would start with 
the default TCP congestion control method,
and must have the capability to switch to 
a new congestion control method as dictated by PM-DCCP above.


==> deployment-old.tex <==
\section{Is Minion Deployable?}

To enable deployment of new transport services atop the minion suite, 
the minion protocols needs to be deployed first.
The changes we need to make to UDP, TCP, and SSL 
in endhosts are described below:
\begin{itemize}
  \item UDP-minion requires no modifications to UDP;
    the transport and/or application atop
    UDP-minion
    need to use port numbers that identify the application endpoints.
    Any additional headers required for new services 
    are encapsulated within the UDP-minion payload.

  \item TCP-minion requires 
    COBS encoding, which can be done in user-space,
    and requires no modifications at the sender-side.
    At the receiver,
    the TCP implementation will need to be modified
    to allow delivery of out-of-order data up to the COBS decoder.
    We have implemented a prototype of such an API extension to TCP in Linux,
    by adding an {\em SO\_UNORDERED} socket option to the TCP socket.

  \item SSL-minion similarly needs the same kernel API extension 
    to TCP at the receive side;
    all other changes required can be implemented
    in the user-space SSL library.
\end{itemize}

Arguments can be
made for the deployability 
of the endhost changes to legacy TCP and SSL for
TCP-minion and SSL-minion,
such as the momentum behind low-latency web transports such as Google's SPDY%
~\cite{spdy}.
Perhaps the strongest arguments for the deployability all minion protocols
are that
none of them requires modifying any middlebox, 
and that
deploying the minion protocols enables deployment
of hitherto undeployable transport services.

\com{
To show that the minion can address
the deployment problem for new transports services,
we need to show that
(i) deployment of minion is a tractable problem, and 
(ii) deploying minion makes it possible to deploy all other transport
services that are promised in new transports (SCTP, SST, DCCP).  We need to
map all three to both UDP and TCP.  UDP encap is generally trivial.
For TCP encap, most of SCTP should be straightforward. 
Some thought is needed to resolve flow control interactions between SST and TCP.
Some thought is needed to resolve partial-/un-reliability with all three protocols.
How to do multihoming?


For the SIGCOMM paper, we should have full protocol reductions for these 
three major protocols on top of the minion suite, and we should build
the three protocols on top of minion to compare against native implementations.
}


==> deployment.tex <==
\subsection{Deploying new transport services}
\label{sec:deployment}

\subsection{Deployment-Impossibility cycles}
(Figure~\ref{f:deployment-impossibility}).
Minion can help in breaking out of these cycles 
(argue more later in conclusion?)

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/deployment-cycles.eps}
\caption{Transport Deployment-Impossibility Cycles}
\label{f:deployment-impossibility}
\end{figure}

\subsection{Why not UDP encapsulation?}

{\bf (XXX condense section.  I don't want to lose much info in this section;  
this is a criticism that we want to address upfront.)}

Given that the demand for new transport services exists,
new transport services are being built and deployed on top of UDP.
Applications such as
Internet telephony (Skype),
video streaming (Adobe's RTMFP for Flash), and
bulk background transport (Bittorrent's uTP),
continue to build their own 
narrowly-focused
transport services over UDP,
and deploy them as part of the application.
To encourage deployment,
transports designed at the IETF
are also employing UDP encapsulation to navigate NATs in the network%
~\cite{tuexen10udp, phelan10dccp}.
While the idea of UDP encapsulation seems seductively simple,
this section discusses
why {\em simple} UDP encapsulation of a new transport
is an inadequate and fragile solution that may
lead to more network encumbrances in the long term.

\subsection{Network Considerations}

While NATs and firewalls often support both TCP and UDP,
they support TCP flows more efficiently
due to the connection state information it provides.
Since NATs cannot precisely determine a UDP session's lifetime,
an application wishing to keep a UDP connection alive
across a NAT or firewall must send keepalive packets
at least every two minutes~\cite{rfc4787},
whereas idle TCP connections require keepalives 
only once every two hours~\cite{rfc5382}.
TCP thus has practical advantages in both bandwidth and power consumption,
especially important for mobile devices,
which are frequently located behind NATs and firewalls
and must keep connections open to listen for incoming notifications.

While simple home NATs and Firewalls
care mainly about port numbers (application endpoint information),
significant parts of the Internet
are behind more sophisticated middleboxes~\cite{rfc3234}
which use TCP connection state information
and assume TCP mechanisms,
such as ack clocking and flow control to achieve their ends.

Stateful Firewalls
maintain and use connection state for filtering traffic and to avoid attacks.
TCP's connection-oriented state machine
makes this information easily available.
Since UDP is connectionless,
Stateful Firewalls
use non-trivial methods
such as 
Deep Packet Inspection (DPI)
and rely on arbitrary timeouts 
and ICMP messages
to determine the state of a session that uses UDP~\cite{northcutt05inside},
thus creating disincentives for operators to allow UDP traffic
into their networks.
Traffic Normalizers~\cite{handley01network}
use detailed information about the TCP state machine to 
thwart network attacks~\cite{marko10using}.
Using UDP leads to heavy use of DPI,
since both Firewalls and Traffic Normalizers
have less information to work with than they would have with TCP,
and they are thus heavily incentivized against allowing UDP traffic.

A new transport that runs on UDP
appears as one among the plethora of extant applications 
that use UDP,
and thus will not be able to navigate broad sledgehammer-like firewall rules 
often found in enterprise firewalls 
that disallow any incoming UDP traffic.

PEPs~\cite{rfc3234}
improve TCP flow performance over 
unconventional network paths,
such as lossy wireless or satellite links,
often by intervening in
TCP mechanisms such as
flow control and ack clocking.
PEPs ignore UDP traffic,
and consequently transports
such as SCTP, SST, and DCCP,
that use TCP-like congestion control mechanisms,
appear to perform poorly on these paths
when run atop UDP,
as we later demonstrate in Section XXX.

All these middleboxes 
need to be made aware of a new transport
for the transport to be deployable and performant in the network
on top of UDP.

\subsection{Yet Another Layer of Multiplexing}
Current proposals~\cite{tuexen10udp, phelan10dccp}
use UDP port numbers merely to demultiplex 
the new transport protocol on top;
the identity of 
the communicating endpoints is hidden away 
in a {\em new} set of port number fields (separate from the UDP port numbers)
embedded in the new transport's protocol headers.
There are thus two sets of port numbers
at the ends:
the UDP port numbers are used to identify
the transport protocol---%
e.g., UDP port 9899 indicates SCTP atop UDP---%
plus the inner transport's SCTP port numbers,
used to identify the application process.
The UDP port numbers are thus 
not usable as a basis for identifying end-applications,
as is commonly done at firewalls.
As a result,
while this solution works for NATs,
Firewalls will need to understand the new protocol's interior headers
to enforce network policy based on port numbers,
and until they are able to, 
administrators will be tempted simply to block the new transport's UDP port.
Thus, where an HTTP session over TCP works,
an HTTP session over SCTP/UDP will not,
even if the firewall's policy is intended to allow web traffic in general.

Future generations of firewalls may eventually understand the 
inner transport and enforce policy 
based on the inner transport's port numbers,
but this simply brings us  back to where we started,
with devices in the network ``understanding''
and allowing traffic from a relatively static
and difficult-to-evolve set of transports atop IP.

Proposals for UDP encapsulation of new transports%
~\cite{tuexen10udp, phelan10dccp}
miss the point that middleboxes need endpoint information,
and encapsulating that information does more harm by 
triggering an arms race with firewall providers.


\subsection{End Host Considerations}

%User-space transports are much easier to deploy
%than kernel-space transports.
Getting user-space transport implementations to perform competitively
with kernel-space implementations
is a non-trivial issue,
and requires much more low-level access than 
is available to most applications 
for close to kernel-level performance~\cite{edwards95experiences}.
Ack-clocked transports,
such as SCTP and SST,
rely on tight timing in transmission and delivery of acks.
Coalescence of ack- and data-delivery,
which results from poor interaction between the ack-clocking of data
and process scheduling on the endhosts,
leads to increased burstiness in the transport~\cite{prasad04effects},
breaking TCP's self-clocking mechanism~\cite{jacobson88congestion},
and resulting in poor performance of TCP-like congestion control%
~\cite{zec02estimating}.
Deploying highly performant transports 
on top of UDP is difficult,
and bandwidth intensive applications
will tend to opt for TCP, 
despite its strait-jacketed service options,
for performance reasons.

Further, new transports that use delay-based congestion control mechanisms
will simply not work in user-space
due to the increased noise in delay signals that comes with
data copying across
the kernel-user boundary 
and with context-switching latency.

\com{
\subsection{Deployment Timescales}
Application requirements and code can and do change more often 
than endhost kernels and code,
which are orders of magnitude faster than changes in the network.
(XXX Quantify through examples. 
changes in killer apps in the last ten years---
web to chat to p2p to games to Internet telephony to Internet video and TV---
changes to network stacks,
changes in the network in the last ten years---ECN deployment?.)
An attempt to deploy a new general-purpose transport protocol,
such as SCTP or SST,
must generally span these three timescales,
which is a very difficult proposition.
}

\subsection{Legacy Comes With Benefits Too}

TCP implementations have 
been maturing and optimized over the past 2-3 decades,
and detailed instrumentation is available for 
learning from and tweaking TCP stacks~\cite{web100, gunawi04deploying}
Offloading parts of the TCP engine
is becoming increasingly important and relevant
~\cite{mogul03tcp},
improving TCP performance and efficiency in high-speed networks.

While other parts have been difficult to get deployed,
variants to the original TCP congestion control~\cite{jacobson88congestion}
are commonplace in general-purpose OS kernels---%
likely in large part due to the fact that congestion control modifications
can usually be deployed without wire-format modifications to TCP.
The major general-purpose Operating Systems---%
MacOSX, Windows7, and Linux---%
all use 
very different congestion control algorithms:
TCP NewReno, Compound TCP, and CUBIC TCP, respectively.
As of kernel v2.6.13, Linux has made it easy for a user 
to choose from a number of congestion control alternatives in the kernel
at run-time%
\footnote{{\em ls /lib/modules/`uname -r`/kernel/net/ipv4/} on a
  Linux-2.6.34 system shows
  an impressive 11 distinct TCP congestion control mechanisms available
  as kernel modules.},
and Mac OSX allows enabling and disabling TCP variants 
such as NewReno and SACK through {\em sysctl}s.
Kernel mechanisms for plugging different
congestion control variants for TCP
already exist in popular Operating Systems,
and where they do not exist yet,
they represent a worthy goal
for kernels that are already dealing with 
diverse network conditions 
ranging from 
low-bandwidth and lossy cellular connectivity on mobile and handheld devices 
to
high-bandwidth connectivity on desktops within enterprise networks.

Legacy TCP thus comes with
a performant and functionality-rich body of software artifacts and tools,
as well as widespread human experience in the industry,
which generally outweighs the costs
of deploying and performance-tuning a new transport atop UDP.


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{itemize}
\item implications to deployment of new transports on the Internet
\item A new datagram service that works through middleboxes is a
  powerful abstraction.
\end{itemize}


==> minion-api.tex <==
\section*{OLD: The Minion API}
\label{sec:minion-api}
Describe the minion API for apps / new transports.


==> minion-suite.tex <==
\section*{OLD: The Minion Suite}
\label{sec:minion-suite}

{\bf(XXX condense description of minions as much as possible.)}

  - goals and overview
  - UDP minion
  - TCP minion
  - SSL minion
  - pulling it all together: the minion API.

\subsection{Goals and Overview}
The goals of the minion suite are as follows:
\begin{itemize}
\item {\em Overcome network inertia:}
	Provide robust, low-latency (out-of-order) forwarding
	of any transport or application PDU
	through middleboxes supporting only TCP or SSL.
\item {\em End-to-end enforcement of transport- and application-neutrality:}
	Provide ability to deploy
    TCP, SCTP, SST, and new transport services atop
    secure end-to-end channels.
\item {\em Substrate-agnostic transport and application operation:}
    A transport or application 
    should not generally {\em need to know} which specific minion it is using
    on a given path.
\end{itemize}

The minion suite employs 
modified forms of
UDP, TCP, SSL, and DTLS 
to provide a low-latency datagram service,
as shown in 
Figure~\ref{f:layers-minion}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-minion.eps}
\caption{The minion protocols and their place in the Tng taxonomy}
\label{f:layers-minion}
\end{figure}

TCP-minion
provides a datagram service
while appearing as TCP on the wire,
with the option of turning congestion control OFF,
and with the option of providing transport layer security through DTLS.
UDP-minion
provides a datagram service
with no congestion control
but exposes endpoint (port number) information.
SSL-minion
provides a secure datagram service
while appearing as SSL on the wire,
with the option of turning congestion control OFF.
Transport protocols,
such as TCP, SCTP, SST, and DCCP,
trimmed to run on the minion suite,
continue to provide their services to applications
in the way they were designed to.

We now describe each of the three minions in more detail.

%\input{tcp-minion}
%\input{ssl-minion}
\input{udp-minion}
\input{minion-api}
%\input{impl}


==> naming.tex <==
\section{Naming and Negotiation}
\label{sec:naming}

How to name an endpoint on a minion?  Port numbers seem insufficient.
One idea: use port numbers as they were; use next-header pointers inside.

How to negotiate and determine minion to use?  One way to think is that 
apps know what the other end will speak---Adobe's RTMFP, as an example
of an app that know precisely what the transport underneath will be.
A more general solution is to use a negotiation service (describe).

This work is ongoing.

==> nego.tex <==
\section{Negotiation}

Two levels of negotiation.  
1.  Negotiate a minion 
2.  Negotiate whether vanilla version or minion version.
TCP/SSL: using a SYN option.
UDP: Header and hash in inner minion header (similar to GUT)


==> overview.tex <==
\section{Overview of the Minion Suite}
\label{sec:overview}
The goals of the minion suite are as follows:
\begin{itemize}
\item {\em Overcome network inertia:}
	Provide robust, low-latency (out-of-order) forwarding
	of any transport or application PDU
	through middleboxes supporting only TCP or SSL.
\item {\em End-to-end enforcement of transport- and application-neutrality:}
	Provide ability to deploy
    TCP, SCTP, SST, and new transport services atop
    secure end-to-end channels.
\item {\em Substrate-agnostic transport and application operation:}
    A transport or application 
    should not generally {\em need to know} which specific minion it is using
    on a given path.
\end{itemize}

The minion suite employs 
modified forms of
UDP, TCP, SSL, and DTLS 
to provide a low-latency datagram service,
as shown in 
Figure~\ref{f:layers-minion}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-minion.eps}
\caption{The minion protocols and their place in the Tng taxonomy}
\label{f:layers-minion}
\end{figure}

TCP-minion
provides a datagram service
while appearing as TCP on the wire,
with the option of turning congestion control OFF,
and with the option of providing transport layer security through DTLS.
UDP-minion
provides a datagram service
with no congestion control
but exposes endpoint (port number) information.
SSL-minion
provides a secure datagram service
while appearing as SSL on the wire,
with the option of turning congestion control OFF.
Transport protocols,
such as TCP, SCTP, SST, and DCCP,
trimmed to run on the minion suite,
continue to provide their services to applications
in the way they were designed to.

In the following three sections,
we now describe each of the three minions in more detail.

\com{
\begin{itemize}
  \item architecture figure and description. brief overview of 
    naming and negotiation components.
  \item figure comparing minion suite to Tng; make architectural points
    about separation of functionality in tng and in minion. Minion
    reuses existing transport protocols, but in explicitly 
    non-traditional roles.
\end{itemize}


Goals:
\begin{itemize}
\item	Overcome old evilness.
	Provide robust, low-latency (out-of-order) packet forwarding
	any transport and application protocols
	from behind proxies allowing only TCP-based
	(e.g., HTTP-only) connectivity.
\item	Overcome new evilness.
	Provide SSL-based mode of operation cryptographically indistinguishable
	at the network level from conventional HTTPS.
\item	End-to-end enforcement of transport- and application-neutrality.
	Run TCP, SCTP, SST, new transports atop.
	Even if network doesn't want you to.
\item	Substrate-oblivious transport and application operation:
	app shouldn't need to know or care which Minion it is running on.
\end{itemize}

}


==> p-works.tex <==
\subsection{Basic Functionality of \utcp}

The experiments in this section
are synthetic microbenchmarks intended to illustrate \utcp's operation,
independently of application-level encodings such as \ucobs or \utls.
These microbenchmarks are not intended to represent
realistic applications or network conditions,
but rather to show \utcp's effects in ``magnified'' settings
to clarify its basic operation.

\paragraph{Receive-side Functionality:}
\begin{figure*}[tbp]
\centering
\includegraphics[width=0.33\textwidth]{figures/works-100msg.eps}
\includegraphics[width=0.33\textwidth]{figures/works-latency.eps}
\includegraphics[width=0.33\textwidth]{figures/works-diffnets.eps}
\caption{
Graphs illustrate the working of \utcp 
and its latency benefits.
Figure (a) shows unordered bytes received at the application with
\utcp, as compared to TCP's ordered delivery.
Figure (b) illustrates \utcp's key benefit to the application:
reduction in application-observed latency.
Figure (c) shows that
\utcp works and performs as well as TCP does 
under different network scenarios, including NATs.}
\label{f:works}
\end{figure*}

Figure~\ref{f:works}(a)
illustrates cumulative bytes delivered by \utcp versus TCP over time,
during a short segment of a bulk transfer,
on a network path with $60$ms roundtrip time (RTT)
and a high $3$\% loss rate.
While bulk transfer does not represent
the type of application \utcp is intended to benefit,
the shape of the lines illustrate \utcp's basic advantage over TCP:
the application keeps receiving new data smoothly from \utcp
even after a packet is lost and must be retransmitted later.

\com{
Under similar network conditions,
{\bf Network conditions are not similar, 
there is a 50ms one way delay and application transmits one packet after 20ms.}
}
Figure~\ref{f:works}(b)
shows a CDF
illustrating the impact of \utcp's unordered delivery
on application-perceived end-to-end latency,
during a fixed-rate transmission
with characteristics similar to a video stream,
across a network with $50$ms one-way delay and a high $2$\% random loss rate.
In this experiment,
the sender transmits $30$MB of data divided into $1448$-byte records,
submitting these records to the send-side TCP stack at $20$ms intervals.
With \utcp, fewer than $3$\%
of the transmitted records are significantly delayed.
Atop TCP, in contrast, over $10$\% of records
are delayed by at least one full RTT,
waiting in the receiving TCP's out-of-order queue
for some sequentially prior packet to be retransmitted.

Figure~\ref{f:works}(c)
shows the progress of a long-running bulk transfer via TCP and \utcp
on two networks:
an emulated network with no middleboxes
($30$ms RTT, $1$\% loss),
and a real $3$Mbps DSL connection
with a residential NAT in the path (roughly 60ms RTT).
At this time-scale the ``notches'' in TCP's progress curve are not visible.
This experiment merely illustrates
that \utcp behaves identically to TCP over time,
and is thus essentially indistinguishable in the network from TCP,
for a given sender-side transmission pattern.

\com{
Graph {\bf (Done. See Figure~\ref{f:works})}:
key point: just show OO delivery happening (microscope).
Synthentic network path, HIGH loss rate.
2 point-line datasets:
(i) plain TCP
(ii) TCPOO.
X axis: time; Y axis: TCP seg start byte no received.
NOTE: This graph is basically an elaboration of the one in the PFLDNeT talk.

Graph {\bf (See Figure~\ref{f:works})}:
latency graph "microbenchmark"?
key point: OO delivery reduces the latency of many packets
Either a CDF or a PDF, not sure which.
Y axis: percentage of segments sent;
X axis: round-trip latency of that segment.
NOTE: state clearly that the workload is entirely synthetic
and designed to make the effects highly pronounced.
Not intended to correspond to any particular real-world scenario or application,
but merely to illustrate "in a microscope" the effect of OO delivery.

Graph {\bf (See Figure~\ref{f:works})}: 
compare operation in different network path scenarios.
key point: it always functions; in common networks we get OO delivery.
shows 3 sets of points: X axis: time; Y axis: TCP seg start byte no received.
(i) 30ms roundtrip, 1Mbps, realistic loss rate
(ii) home to FandM (NAT), realistic loss rate
(iii) through Cisco PEP w/ TCP termination/normalization,
NOTE: This graph focuses on the TCP stack modification,
independently of all user-space encoding/usage issues.
}
%\begin{figure}[tbp]
%\centering
%\includegraphics[width=0.49\textwidth]{figures/works-hnw-time-vs-sn-1.ps}
%\includegraphics[width=0.49\textwidth]{figures/works-snw-time-vs-sn-1.ps}
%\caption{Figures show that \utcp works and performs as well as TCP 
%on networks with different middlebox. The experimental scenarios have:
%(a) No middleboxes between the endhosts;
%(b) One end behind a NAT; and
%(c) Two PEPs between the endhosts.}
%\label{f:works-3}
%\end{figure}



==> sctp.tex <==
\subsection{A Poor Man's SCTP}
\label{sec:sctp}

SCTP~\cite{rfc4960}
is a recent transport protocol,
that,
similar to TCP,
provides
a fully reliable and congestion-controlled flow
with receiver-driven flow control.
In addition,
SCTP provides three services to an application:
\begin{enumerate}
\item {\em message-boundary preservation}, which ensures that 
a sending application's message-boundaries
are maintained and faithfully reproduced
to the receiving application,
even if the message spans several transport segments;

\item {\em multi-streaming}, by which an application can
create multiple logically-independent and ordered data streams
within a single SCTP connection,
avoiding head-of-line blocking across independent data streams
within the SCTP connection,
while sharing congestion state and 
data loss detection and recovery
across these data streams; and

\item {\em unordered message delivery}, 
which allows a sending application to indicate messages
to be delivered to the receiving application
without regard to the order of their reception 
at the receiving transport.

\end{enumerate}

Transparent to the application,
the most important feature that
SCTP offers is multi-homing---%
an SCTP connection can span several IP addresses
at each endhost,
which allows the connection to
be tolerant to network failures.

\subsubsection{Designing PM-SCTP}

{\em Message boundary preservation, and Unordered delivery:} 
Both \ucobs and \utls
provide message-boundary preservation 
and unordered but reliable message delivery.
PM-SCTP simply \ucobs or \utls
to provide these services to the application.
PM-SCTP is thus defined as a shim between
the application and \ucobs or \utls.

{\em Multi-streaming:} 
An SCTP sender fragments
application messages
into independent {\em chunks} which are encapsulated in {\em chunk headers};
several chunks, are gathered into 
SCTP segments that are then transmitted over IP.
This design allows an SCTP sender 
to gather chunks from different
SCTP streams into a single SCTP segment,
thus multiplexing transmission across the SCTP streams.
The SCTP receiver gathers received chunks and re-assembles them
into messages before delivering them to the receiving application.

A PM-SCTP sender generates SCTP chunks similarly,
but instead of gathering these chunks into an SCTP segment,
PM-SCTP directly transmits this chunk
over \ucobs or \utls.
The PM-SCTP receiver receives these chunks
from \ucobs or \utls interface,
possibly out-of-order;
the PM-SCTP receiver,
as the SCTP receiver,
can manage these out-of-order chunks independently.

To implement multi-streaming,
the chunk header
that SCTP (and PM-SCTP) employs
carries stream ID and stream sequence number 
required for the receiving SCTP (and PM-SCTP)
to deliver messages to the application on a stream independent
of the data received on the other streams.

{\em Multihoming}:
%SCTP's native multihoming
%uses 
PM-SCTP can make use of multiple TCP connections
to approximate the fault tolerance that SCTP multi-homing provides;
similar ideas have been explored in the past~\cite{ekwall02robust}.
Multipath TCP (MPTCP), a new IETF protocol under development~\cite{ford10tcp}
that adds SCTP-like multi-homing and fault tolerance 
to TCP,
can also eventually provide multi-homing underneath PM-SCTP.

\subsubsection{A Prototype PM-SCTP Implementation}
We implemented a prototype of PM-SCTP as a userspace library
on top of \ucobs 
in about XXX lines of C code.
Our implementation
does not provide multi-homing yet,
but it offers
all the other SCTP services to applications.


%\subsubsection{Benefits with a web workload}
%Experiments showing multistreaming benefits?

%\subsubsection{Benefits with multihoming}


==> services.tex <==
\section{New Transport Services}
\label{sec:services}

Over the past decade,
new Internet transports have been developed
in response to applications' changing needs,
providing a variety of new services
beyond those offered by TCP\@.
This paper focuses on only one such service,
unordered delivery,
in part because it is a feature that applications
{\em cannot} implement for themselves atop TCP.
The TCP stack's standard in-order delivery semantics
by definition prevent the application
from learning anything about out-of-order segments
until all prior gaps are filled,
so the standard TCP stack in essence denies the application
precisely the information it would need to implement out-of-order delivery.

Having addressed TCP's lack of out-of-order delivery support, however,
we see an important follow-up question:
given all of the {\em other} new services
that other transports such as DCCP, SCTP, and SST provide,
which of those features are ``fundamental'' to the transport layer,
and which could potentially be implemented by applications
atop an out-of-order delivery substrate such as \utcp?
As a thought exercise,
we now explore this question
by considering a few possible abridged,
but immediately deployable,
versions---``Poor Man's'' versions---of
other recent transport protocols.

\subsection{Building New Services Atop \utcp}
\label{sec:building}
Beyond the services TCP already provides,
additional services that have proven of interest in new transports
include:

\begin{itemize}
\item {\em Message-boundary preservation}:
Both \ucobs and \utls
ensure that 
a sending application's message-boundaries
are maintained and faithfully reproduced
to the receiving application,
even if the message spans several transport segments,
even if the transport segments are re-segmented in the network,
and even if the message is received out-of-order.

\item {\em Unordered message delivery}:
\ucobs and \utls 
are designed and built atop \utcp
to provide precisely this service,
as described extensively earlier in this paper.

\item {\em Multistreaming}:
Applications often seek to
create logically independent data streams
within a single transport connection,
to avoid head-of-line blocking across independent data streams
within the connection;
for eg.,
web browsers
are constantly increasing the number of parallel TCP connections
that they use to download a webpage from a webserver,
so as to allow parallelism in load and display times for 
the independent components of webpages.
\ucobs and \utls 
provide independent message delivery;
we simply insert a minimal ``stream header'' that identifies 
a message as belonging to a particular application stream,
and indicates its position in the stream;
multistreaming can thus be built 
using independent and unordered  message delivery as a building block.

\item {\em Multihoming and Mobility Management}:
Multiple \utcp connections
can be utilized
to provide connectivity via multihoming
and for session mobility;
similar ideas have been explored in the past~\cite{ekwall02robust}.
Unordered message delivery in \ucobs and \utls 
allows for signaling messages to be transmitted 
within a \utcp connection
that can be effectively utilized for 
connection migration and mobility.
Multipath TCP (MPTCP), a new IETF protocol under development~\cite{ford10tcp}
that adds multi-homing and fault tolerance to TCP,
can also eventually natively provide multihoming 
and mobility management capabilities
to \utcp.
\end{itemize}


\subsection{``Poor Man's'' New Transports}

Despite the demand for new transport services,
it is practically impossible to deploy any new transport protocol
since new transports require support not only at the endpoints
but also in middleboxes.
As a way out of this logjam,
we now consider
Poor Man's versions of two new transport protocols---%
SCTP~\cite{rfc4960}, and DCCP~\cite{rfc4340}---%
%, and SST~\cite{ford07structured}.
and a congestion sharing mechanism---%
Balakrishnan et al's Congestion Manager~\cite{balakrishnan99integrated}---%
that can be built atop 
\utcp, \ucobs and/or \utls,
but could hitherto not be built atop TCP due to its strictly ordered delivery.

\subsubsection{Why Build Transport Protocols Atop \utcp?}

There are three major benefits to building a transport atop \utcp:
\begin{enumerate}

\item A Poor Man's transport appears as TCP or TLS on the wire, 
and thus does not require any middlebox in the network to adapt.
Figure~\ref{f:tcp-middleboxes} 
shows how 
middleboxes in the modern Internet
interact with TCP,
and how the Poor Man's transports can remain network-compatible 
by stacking atop \utcp\footnote{
Middleboxes that perform Deep Packet Inspection (DPI)
are generally frequently updated
to keep up with changing application signatures.
and can be updated
to decode COBS encoded app data
at marginal additional CPU cost.}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/tcp-middleboxes.eps}
\caption{Network devices interact with the transport and \utcp
enables new transport services for applications
while remaining compatible with network.}
\label{f:tcp-middleboxes}
\end{figure}

\item A Poor Man's transport can be deployed as a userspace library, 
and application developers can build and deploy new transports 
within applications themselves atop \utcp.

\item Poor Man's transports can be designed assuming \utcp
and deployed in applications without {\em requiring} \utcp at either
endhost, as discussed in Section~\ref{sec:usage};
\utcp is an endhost-local modification that impacts performance,
but does not impact TCP interoperability.
\end{enumerate}

The strength of \utcp-based transports 
is that they are entirely backward-compatible with the network,
and whereas they may not be able to span the entire gamut of
new possible transport services and features,
they make up for wide scope by being immediately deployable.

\subsubsection{A Poor Man's SCTP}
SCTP~\cite{rfc4960}
is a recent transport protocol,
that,
similar to TCP,
provides
a fully reliable and congestion-controlled connection
with receiver-driven flow control.
In addition,
SCTP provides
message-boundary preservation,
multistreaming,
and multihoming
to an application.
%An SCTP extension provides
%message-level partial reliability~\cite{rfc3758}.
Our {\em Poor Man's SCTP (PM-SCTP)}
can provide reasonable approximations,
if not semantically exactly the same,
services atop \utcp,
as described in Section~\ref{sec:building}.

We have implemented a prototype of 
PM-SCTP as a userspace library
on top of \ucobs
in about $300$ lines of C code~\cite{cloc-153}.
Our implementation
does not provide multihoming yet,
but it offers
all the other SCTP services to applications.

\subsubsection{A Poor Man's DCCP}
The Datagram Congestion Control Protocol (DCCP)~\cite{rfc4340, kohler06dccp}
was designed for streaming and voice/video-conferencing applications,
and it provides a congestion-controlled unreliable datagram service
with the ability to negotiate congestion control mechanisms at 
flow setup time.

Our first approximation
of a {\em Poor Man's DCCP (PM-DCCP)} is simple:
by definition,
\ucobs and \utls
provide the semantic equivalent of
DCCP with TCP-like congestion control~\cite{rfc4341},
with the difference that DCCP does not provide reliability.

As a further refinement, with several 
congestion control options available for TCP in most 
popular Operating Systems\footnote{
Linux-2.6.34 provides an impressive $11$ congestion control
modules for TCP},
PM-DCCP 
can start the \utcp connection with the default 
TCP-NewReno or TCP-SACK congestion control
and can negotiate,
above \utcp,
the congestion control option to be used
for the rest the connection.
This negotiated congestion control option
can then be set at the endhosts
using a \verb|setsockopt()|
or equivalent mechanism.
This negotiability requires 
that TCP stacks have the capability to switch  
congestion control schemes during an active connection,
which requires some thought but seems tractable.

\subsubsection{A Poor Man's Congestion Manager}
\label{sec:cm}
The Congestion Manager~\cite{balakrishnan99integrated}
provides a framework by which all application flows 
between two endhosts 
share congestion state,
irrespective of the transport protocol they use.
Since \ucobs and \utls offer
a congestion-controlled and reliable datagram interface,
we can also use them as the basis for 
a {\em Poor Man's Congestion Manager (PM-CM)}
that provides aggregate congestion control to
\utcp-based transports above.
A PM-CM shim atop \ucobs or \utls
introduces a thin header, 
similar to the CM,
to multiplex and demultiplex
different application flows above.

%\input{sctp}
%\input{sst}
%\input{dccp}
%\input{cm}
\com{
Discuss RUTS requirements? ( We should at least state that these
requirements have been around for a while, and we can see how many of
them we can address with uTCP.  See
\url{http://www.ietf.org/proceedings/43/43rd-ietf-98dec-142.html})

- shared congestion control among multiple application streams
- record boundaries
- no strict ordering
- Quick setup, data in first RTT.  
once connection is established,
stream setup and teardown can be done in application space; 
use SST techniques on top of minions.
- MPTCP will eventually allow for connection migration and failover.
Even if not, multiple connections can be used under minions 
for multihoming, and SCTP multihoming can be incorporated into Semantic SCTP.

- mapping to the Congestion Manager? (``A poor man's congestion manager'')
}

\com{
\subsection{Limitations of \utcp-based Services}

There are fundamental limitations
to the range of services that can be stacked atop \utcp
that arise due to the design premise that they must be 
entirely wire-compatible with TCP.

\begin{itemize}
\item 
SCTP's design allows it to be extended 
to support partial reliability~\cite{rfc3758},
whereas segment-level partial reliability
is not possible with PM-SCTP or any other protocol that is stacked atop \utcp.
Similarly, TFRC congestion control used by DCCP~\cite{rfc3448}
requires fundamentally different feedback mechanisms 
from the receiver to the sender of the data flow;
such modifications are beyond what is possible with \utcp.
\end{itemize}
}


==> sst.tex <==
\subsection{A Poor Man's SST (PM-SST)}
\label{sec:sctp}

\subsubsection{Designing PM-SST}
Show SST API and mapping (paths) to Minion API.
Briefly show how services are offered, focus on forking of streams and 
receiver-driven per-stream flow control.

%\subsection{Experiments}
%Web browsing with receiver-side control of stream priority---
%e.g., shut out parts of web page that are not being displayed.


==> taxonomy.tex <==
\subsection{Transport Protocols Vs. \\The brave new world}
\label{sec:taxonomy}

(XXX need to change figures to show transport layer functions 
instead of sub-layers.)

We first develop a taxonomy of transport functions, 
and examine the
interactions between middleboxes in the modern Internet
and the traditionally-end-to-end transport layer.
This taxonomy builds on previous work~\cite{ford08breaking},
and extends it to include security functions.
We first factor out functional components 
within the traditional transport layer into four sub-layers,
as previously proposed in \Tng~\cite{ford08breaking}.
Starting from the sub-layer immediately above the network layer, 
these are:
\begin{description}
\item [The Endpoint Layer] factors out communication endpoint information---%
  port numbers in the current Internet architecture---%
  that policy-enforcing middleboxes such as firewalls, NATs,
  and traffic shapers require for operation;
\item [The Flow Regulation Layer]  
  factors out congestion control and other functions
  that may require network interaction
  for purposes of adapting to network heterogeneity;
\item [The Semantic Layer] 
  factors out application-oriented services
  such as end-to-end reliability and ordering; and
\item [The Isolation Layer]
  is an optional layer,
  traditionally above the Semantic Layer,
  which provides end-to-end cryptographic security
  via protocols such as TLS~\cite{rfc5246} and DTLS~\cite{rfc4347}.
\end{description}

Figure~\ref{f:layers-middleboxes} shows how middleboxes interact
with and interpose on different transport layer components.
NATs and Firewalls 
care about port numbers and application endpoint information,
Performance Enhancing Proxies (PEPs)~\cite{rfc3234} 
care about congestion control,
Traffic Normalizers~\cite{handley01network}
use detailed information about the TCP state machine to 
thwart network attacks,
and Corporate Firewalls are increasingly starting to employ
SSL proxies as trusted intermediaries to
prevent attacks through encrypted channels~\cite{marko10using}.
Stateful Firewalls
maintain and use connection state for filtering traffic and to avoid attacks.
Traffic Normalizers~\cite{handley01network}
use detailed information about the TCP state machine to 
thwart network attacks~\cite{marko10using}.

(XXX change figure to remove discussion of SSL proxies, 
and of corp firewalls extending into isolation layer.
Not needed since that is not a technical problem that we can fix here.)


\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-middleboxes.eps}
\caption{A taxonomy of Transport functions showing how middleboxes interact with the Transport}
\label{f:layers-middleboxes}
\end{figure}


Figure~\ref{f:layers-current-transports} 
shows how transports are designed and deployed on the Internet,
and a comparison with Figure~\ref{f:layers-middleboxes}
shows how new transports conflict with legacy middleboxes.

\begin{figure}[htb]
\centering
\includegraphics[width=0.49\textwidth]{figures/layers-current-transports.eps}
\caption{Transport protocols in the Tng taxonomy}
\label{f:layers-current-transports}
\end{figure}

\subsection{New transport services are in demand}
- Demonstrate that new transport services are in demand by apps.
- Show examples of new transport services that are being deployed
  as part of app libraries, how they are in private silos, and 
  how they are reinventing wheels. uTP services?, RTMFP has multistreaming 
  and high-speed cong control. Other examples:  Quake, HTML5 and HyBi.




==> udp-minion.tex <==
\subsection{A UDP Minion}
\label{sec:udp-minion}

Perhaps the simplest of the minions,
UDP-minion is a UDP encapsulation 
of the transport or application protocol,
but with one key difference from current proposals%
~\cite{tuexen10udp, phelan10dccp}---%
UDP-minion does not add an additional point of demultiplexing.
While the recent proposal for Generic UDP Tunneling (GUT)%
~\cite{manner10generic} 
suggests such a possibility,
our UDP-minion deliberately avoids a UDP demultiplexer 
followed by an upper layer demultiplexer,
in keeping with Feldmeier~\cite{feldmeier90multiplexing} 
and Tennenhouse~\cite{tennenhouse89layered}.

\com{
The goal of UDP-minion is not passage through obscurity.
We argue that 
such a design only leads to more aggressive use of DPI by
network operators,
and so, UDP-minion leaves
the application endpoints in the clear.
}
